Controlling a Markov Decision Process with an Abrupt Change in the Transition Kernel

We consider the control of a Markov decision process (MDP) that undergoes an abrupt change in its transition kernel (mode). We formulate the problem of minimizing regret under control-switching based on mode change detection, compared to a mode-observing controller, as an optimal stopping problem. Using a sequence of approximations, we reduce it to a quickest change detection (QCD) problem with Markovian data, for which we characterize a state-dependent threshold-type optimal change detection policy. Numerical experiments illustrate various properties of our control-switching policy.

==> approx_regret.tex <==
% \section{Expected Regret}
\iffalse
From the prior section, we have that the following problem 
\begin{equation}\label{eq:EDD_PFA_lagr}
    \min_{\tau\in \Scal}\,\EDD(\tau) + \bar{\lambda}\cdot\PFA(\tau)
\end{equation}
is equivalent to the problem 
\begin{equation}\label{eq:EDD_EFAT_lagr}
    \min_{\tau\in \Scal}\,\EDD(\tau) + \lambda\cdot\EFAT(\tau),
\end{equation}
when $\bar{\lambda} = \lambda/\rho$. Thus, the threshold structure of the optimal policy for \eqref{eq:EDD_PFA_lagr} carries over to the optimal policy for \eqref{eq:EDD_EFAT_lagr}.  \\~\\
%
Note that \eqref{eq:EDD_PFA_lagr} can be seen as the Lagrangian relaxation of the problem 
\begin{equation}\label{eq:EDD_PFA}
    \begin{split}
        \min_{\tau\in\Scal}&\quad \EDD(\tau)\\
        \text{s.t.}&\quad \PFA(\tau)\leq \alpha.
    \end{split}
\end{equation}
It can be shown that there exist a $\bar{\lambda}$ such that the optimal stopping procedure to \eqref{eq:EDD_PFA_lagr} is optimal for \eqref{eq:EDD_PFA} as well. \\~\\
%
The (optimal) thresholding structure described in Theorems \ref{thm:thresh_finite} and \ref{thm:thresh_infinite} is known as the Shiryaev procedure. In the case of i.i.d. observations prior to and following the change, the following result is know. 

\begin{theorem}
Let, conditioned on $\Gamma=k$, the observations $X_1,\dots,X_{k-1}$ be i.i. with pdf $f_0(x)$ and let $X_k,X_{k+1},\dots$ be i.i.d with pdf $f_1(x)$. Further, let the prior distribution of the change point $\Gamma$ be geometric with parametr $\rho$. Suppose that 
\begin{equation}
    0<D(f_0,f_1)<\infty\quad \text{and}\quad 0<D(f_1,f_0)<\infty,
\end{equation}
where $D(f_0,f_1)$ and $D(f_0,f_1)$ give the KL information number between $f_0$ and $f_1$. As $\alpha\to0$, we have that 
\begin{equation}
    \inf_{\tau\in\Scal(\alpha)}\,\,\EDD(\tau)
\end{equation}
\end{theorem}
\fi
% \section{Optimal Stopping Time Formulation}
% Let $\{X'_t\}$ denote the process associated with mode observing controller. Note that $X_t = X'_t$ for $t\leq \min\{\tau,\Gamma\}$. The random cost of stopping at time $\tau=n$ is
% \begin{equation}\nonumber
%     \begin{split}
%         % &Y_n = \mathds{1}_{\{n<\Gamma\}}\Bigg(\sum_{t=0}^{n-1}\gamma^t\left[c(X_t,\pi_1(X_t))-c(X'_t,\pi_1(X'_t))\right]\\
%         % &\hspace{0.75in}+ \sum_{t=n}^{\Gamma-1}\gamma^t\left[c(X_t,\pi_2(X_t)) - c(X'_t,\pi_1(X'_t))\right]\\
%         % &\hspace{0.75in}+ \sum_{t=\Gamma}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)\\
%         % &\hspace{0.25in}+ \mathds{1}_{\{n> \Gamma\}}\Bigg(\sum_{t=0}^{\Gamma-1}\gamma^t\left[c(X_t,\pi_1(x_t)) - c(X'_t,\pi_1(X'_t))\right]\\
%         % &\hspace{0.75in}+ \sum_{t=\Gamma}^{n-1}\gamma^t\left[c(X_t,\pi_1(X_t))-c(X'_t,\pi_2(X'_t))\right]\\
%         % &\hspace{0.75in}+ \sum_{t=n}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)\\
%     %%%%%%
%         &Y_n = \mathds{1}_{\{n<\Gamma\}}\Bigg(\sum_{t=n}^{\Gamma-1}\gamma^t\left[c(X_t,\pi_2(X_t)) - c(X'_t,\pi_1(X'_t))\right]\\
%         &\hspace{0.6in}+ \sum_{t=\Gamma}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)\\
%         &\hspace{0.1in}+ \mathds{1}_{\{n> \Gamma\}}\Bigg( \sum_{t=\Gamma}^{n-1}\gamma^t\left[c(X_t,\pi_1(X_t))-c(X'_t,\pi_2(X'_t))\right]\\
%         &\hspace{0.6in}+ \sum_{t=n}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)\\
%         &\hspace{0.1in}\equiv C^{\FA}_n +C^{\D}_n,
%     \end{split}
% \end{equation}
% where $C^{\FA}_n$ and $C^{\D}_n$ denote the random costs associated with false alarm and delay, respectively, when stopping at time $n$.\\~\\
% Let $\Pcal$ denote the set of distributions over the state space $\Xset$. For $Q\in\Pcal$, $J^m_{Q}(\pi_i;P_j)$ denotes the expected $m$ step horizon cost, given that the initial state is distributed according to $Q$. If the initial state $X$ is given, we write $J^m_{X}(\pi_i;P_j)$. In either case, when $m=\infty$, we drop the superscript, e.g. $J_{Q}(\pi_i,P_j) := J^{\infty}_{Q}(\pi_i,P_j)$. Lastly, we denote as %$P^{m,i|j}_{X} = P(X,\pi_i,j,m)$ 
% $P^{m,i|j}_{X}$ the $m$ step probability distribution, given that the system started in state $X$, and policy $\pi_i$ is used in mode $j$. 
\subsubsection{Expected False Alarm Cost}
Conditioning on $X_0^n$, the expected false alarm regret is 
\begin{equation}
\label{eq:cond_exp_FA_cost}
    \begin{split}
        &\E\left[C^{\FA}_n|X_0^n\right]=\\
        & \E\Bigg[\mathds{1}_{\{n<\Gamma\}}\Bigg( \sum_{t=n}^{\Gamma-1}\gamma^t\left[c(X_t,\pi_2(X_t)) - c(X'_t,\pi_1(X'_t))\right]\\
        &\hspace{0.25in}+ \sum_{t=\Gamma}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)|X^n_0\Bigg].\\
        %&= P(n<\Gamma|X^n_0)\E\left[\gamma^n\left(J^{\Gamma-n}_{X_n}(\pi_2;P_1) - J^{\Gamma-n}_{X_n}(\pi_1;P_1)\right) + \gamma^{\Gamma}\left(J_{P^{\Gamma-n,X_n}_{2|1}}(\pi_2;P_2) - J_{P^{\Gamma-n,X_n}_{2|2}}(\pi_2;P_2)\right)|X_n\right].
        % &= \E\Bigg[\mathds{1}_{\{n<\Gamma\}}\left( \sum_{t=n}^{\Gamma-1}\gamma^tc(X_t,\pi_2(X_t)) +\sum_{t=\Gamma}^{\infty}\gamma^tc(X_t,\pi_2(X_t))\right)|X^n_0\Bigg]\\
        % &\qquad\qquad\qquad\qquad - \E\Bigg[\mathds{1}_{\{n<\Gamma\}}\left( \sum_{t=n}^{\Gamma-1}c(X'_t,\pi_1(X'_t))+\sum_{t=\Gamma}^{\infty}c(X'_t,\pi_2(X'_t))\right)|X^n_0\Bigg]\\
        % &= \E\Bigg[\mathds{1}_{\{n<\Gamma\}}\left( \sum_{t=n}^{\Gamma-1}\gamma^tc(X_t,\pi_2(X_t)) +\sum_{t=\Gamma}^{\infty}\gamma^tc(X_t,\pi_2(X_t))\right)|X^n_0\Bigg]\\
        % &\qquad\qquad\qquad\qquad - P(n<\Gamma|X^n_0)\E\left[J^{\Gamma}_{X_n}(\pi_1;P_1) + J_{P^{\Gamma,X_n}_{1|1}}(\pi_2;P_2)|X^n_0\right]
        % &= \mathds{1}_{\{n<k\}}\E\left[\sum_{t=0}^{n-1}\gamma^tc(x_t,\pi_1(x_t)) + \sum_{t=n}^{k-1}\gamma^tc(X_t,\pi_2(X_t)) + \sum_{t=k}^{\infty}\gamma^tc(X_t,\pi_2(X_t))|X^n_0,\Gamma=k\right]\\
        % &= \mathds{1}_{\{n<k\}}\left(\gamma^{n}\E\left[J^{k-n}_{x_n}(\pi_2;P_1) - J^{k-n}_{x_n}(\pi_1;P_1)\right] + \gamma^k\E\left[J_{P^{k-n,x_n}_{2|1}}(\pi_2;P_2) - J_{P^{k-n,x_n}_{1|1}}(\pi_2;P_2)\right]\right)
    \end{split}
\end{equation}
For the first part of \eqref{eq:cond_exp_FA_cost}, corresponding to the time between the change declaration and actual mode change, we have 
\begin{equation}\label{eq:FA_calc_1}
    \begin{split}
        &\E\Bigg[\mathds{1}_{\{n<\Gamma\}}\left( \sum_{t=n}^{\Gamma-1}\gamma^t\left[c(X_t,\pi_2(X_t)) - c(X'_t,\pi_1(X'_t))\right]\right)|X^n_0\Bigg]\\
        &\overset{(a)}{=}\gamma^n\sum_{k=1}^{\infty}\E\Bigg[\mathds{1}_{\{n<\Gamma\}} \Bigg(\sum_{t=n}^{\Gamma-1}\gamma^{t-n}[c(X_t,\pi_2(X_t))\\
        &\hspace{0.75in}- c(X'_t,\pi_1(X'_t))]|X^n_0,\Gamma=k\Bigg]\Bigg)P(\Gamma=k|X^n_0)\\
        &\overset{(b)}{=}\gamma^n\sum_{k=1}^{\infty}\mathds{1}_{\{n<k\}}\E\Bigg[ \sum_{t=n}^{k-1}\gamma^{t-n}[c(X_t,\pi_2(X_t))\\
        &\hspace{0.75in}- c(X'_t,\pi_1(X'_t))]|X^n_0,\Gamma=k\Bigg]P(\Gamma=k|X^n_0)\\
        &\overset{(c)}{=}\gamma^n\E\left[\mathds{1}_{\{n<\Gamma\}}\left(J^{\Gamma-n}_{X_n}(\pi_2;P_1) - J^{\Gamma-n}_{X_n}(\pi_1;P_1)\right)|X^n_0\right],
    \end{split}
\end{equation}
Equality $(a)$ follows from rewriting the conditional expectation in terms of a sum over the conditional distribution of $\Gamma$, given $X^0_n$, and moving the constant term $\gamma^n$ outside of the expectation and summation. Equality $(b)$ follows from applying the inner conditioning to $\Gamma$, and observing that the resulting indicator function $\mathds{1}_{\{n<k\}}$ becomes a constant with respect to the inner conditional expectation. Equality $(c)$ follows from the definition of conditional expectation.
\\~\\
%
The second part of \eqref{eq:cond_exp_FA_cost}, corresponding to the time following the mode change can be rewritten as
\begin{equation}\label{eq:FA_calc_2}
    \begin{split}
        &\E\Bigg[\mathds{1}_{\{n<\Gamma\}}\left(\sum_{t=\Gamma}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\right)|X^n_0\Bigg]\\
        &=\sum_{k=1}^{\infty}\E\Bigg[\mathds{1}_{\{n<k\}}\Bigg(\sum_{t=k}^{\infty}\gamma^t[c(X_t,\pi_2(X_t))\\
        &\hspace{0.75in}-c(X'_t,\pi_2(X'_t))]\Bigg)|X^n_0,\Gamma=k\Bigg]P(\Gamma=k|X^n_0)\\
        &=\sum_{k=1}^{\infty}\mathds{1}_{\{n<k\}}\gamma^{k}\E\Bigg[\sum_{t=k}^{\infty}\gamma^{t-k}[c(X_t,\pi_2(X_t))\\
        &\hspace{0.75in}-c(X'_t,\pi_2(X'_t))]|X^n_0,\Gamma=k\Bigg]P(\Gamma=k|X^n_0)\\
        &= \E\left[\mathds{1}_{\{n<\Gamma\}}\gamma^{\Gamma}\left(J_{P^{\Gamma-n,2|1}_{X_n}} - J_{P^{\Gamma-n,1|1}_{X_n}}\right)|X^n_0\right].
        % &=\sum_{k=1}^{\infty}\gamma^{k}\E\Bigg[\left(\sum_{t=k}^{\infty}\gamma^{t-k}\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\right)|X^n_0,\Gamma=k\Bigg]P(\Gamma>n,\Gamma=k|X^n_0)\\
        % &=P(\Gamma>n|X^n_0)\sum_{k=1}^{\infty}\gamma^{k}\E\Bigg[\left(\sum_{t=k}^{\infty}\gamma^{t-k}\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\right)|X^n_0,\Gamma=k\Bigg]P(\Gamma=k|X^n_0,\Gamma>n)\\
        % &=P(\Gamma>n|X^n_0)\sum_{k=1}^{\infty}\gamma^{k}\left(J_{P^{k-n,X_n}_{2|1}}(\pi_2;P_2) - J_{P^{k-n,X_n}_{1|1}}(\pi_2;P_2)\right)P(\Gamma=k|X^n_0,\Gamma>n)\\
        % &=P(\Gamma>n|X^n_0)\E\left[\gamma^{\Gamma}\left(J_{P^{k-n,X_n}_{2|1}}(\pi_2;P_2) - J_{P^{k-n,X_n}_{1|1}}(\pi_2;P_2)\right)|X^n_0,\Gamma>n\right].
    \end{split}
\end{equation}
The steps in \eqref{eq:FA_calc_2} follow from the same reasoning as in \eqref{eq:FA_calc_1}, the only difference being that the $\gamma^k$ factor must remain inside the summation. 
    % We have that 
    % \begin{equation}
    %     \begin{split}
    %         P(\Gamma>n,\Gamma=k|X^n_0) &= \frac{P(\Gamma>n,\Gamma=k,X^n_0)}{P(X^n_0)}\\
    %         &= \frac{P(\Gamma=k|\Gamma>n,X^n_0)P(\Gamma>n,X^n_0)}{P(X^n_0)}\\
    %         &=P(\Gamma=k|\Gamma>n,X^n_0)P(\Gamma>n|X^n_0)\\
    %         &=\frac{P(\Gamma=k,\Gamma>n,X^n_0)}{P(\Gamma>n,X^n_0)}P(\Gamma>n|X^n_0)\\
    %         &=\frac{P(X^n_0|\Gamma=k,\Gamma>n)P(\Gamma=k,\Gamma>n)}{P(X^n_0|\Gamma>n)P(\Gamma>n)}P(\Gamma>n|X^n_0)\\
    %         &=\frac{P(\Gamma=k,\Gamma>n)}{P(\Gamma>n)}P(\Gamma>n|X^n_0)\\
    %         % &=P(\Gamma=k|\Gamma>n)P(\Gamma>n|X^n_0)\\ 
    %         % &=P(\Gamma=k-n)P(\Gamma>n|X^n_0).
    %         % &= \frac{P(\Gamma>n,\Gamma=k,X^n_0)}{P(\Gamma>n,X^n_0)}P(\Gamma>n|X^n_0)\\
    %         % &= \frac{P(X^n_0|\Gamma>n,\Gamma=k)P(\Gamma>n,\Gamma=k)}{P(X^n_0|\Gamma>n)P(\Gamma>n)}P(\Gamma>n|X^n_0)\\
    %         % &= \frac{P(\Gamma>n,\Gamma=k)}{P(\Gamma>n)}P(\Gamma>n|X^n_0)\\
    %         % &= P(\Gamma=k|\Gamma>n)P(\Gamma>n|X^n_0)\\
    %         &= P(\Gamma=k-n)P(\Gamma>n|X^n_0).
    %     \end{split}
%     % \end{equation}
%     Therefore, continuing 
%         \begin{equation}\begin{split}
%         &\E\Bigg[\mathds{1}_{\{n<\Gamma\}}\left(\sum_{t=\Gamma}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\right)|X^n_0\Bigg]\\
%         &=P(\Gamma>n|X^n_0)\sum_{k=1}^{\infty}\gamma^{k}\E\Bigg[\left(\sum_{t=k}^{\infty}\gamma^{t-k}\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\right)|X^n_0,\Gamma=k\Bigg]P(\Gamma=k-n)\\
%         &=P(\Gamma>n|X^n_0)\sum_{k=1}^{\infty}\gamma^{k}\left(J_{P^{k-n,X_n}_{2|1}}(\pi_2;P_2) - J_{P^{k-n,X_n}_{1|1}}(\pi_2;P_2)\right)P(\Gamma=k-n)\\
%         &=P(\Gamma>n|X^n_0)\sum_{k=n+1}^{\infty}\gamma^{k}\left(J_{P^{k-n,X_n}_{2|1}}(\pi_2;P_2) - J_{P^{k-n,X_n}_{1|1}}(\pi_2;P_2)\right)P(\Gamma=k-n)
%         % &=P(\Gamma>n|X^n_0)\sum_{k=n+1}^{\infty}\gamma^k\E_{\substack{X_{t+1}\sim P_2(\cdot|X_t,\cdot)\\X_0\sim P^{k-n,X_n}_{2|1}\\X'_{t+1}\sim P_2(\cdot|X'_t,\cdot)\\X'_0\sim P^{k-n,X_n}_{1|1}}}\Bigg[\sum_{t=0}^{\infty}\gamma^{t}\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg]P(\Gamma=k-n)\\
%         % &=P(\Gamma>n|X^n_0)\sum_{k=1}^{\infty}\gamma^{k+n}\E_{\substack{X_{t+1}\sim P_2(\cdot|X_t,\cdot)\\X_0\sim P^{k,X_n}_{2|1}\\X'_{t+1}\sim P_2(\cdot|X'_t,\cdot)\\X'_0\sim P^{k,X_n}_{1|1}}}\Bigg[\sum_{t=0}^{\infty}\gamma^{t}\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg]P(\Gamma=k)\\
%         % &=P(\Gamma>n|X^n_0)\sum_{k=1}^{\infty}\gamma^{k+n}\E_{\substack{X_{t+1}\sim P_2(\cdot|X_t,\cdot)\\X_0\sim P^{k,X_n}_{2|1}\\X'_{t+1}\sim P_2(\cdot|X'_t,\cdot)\\X'_0\sim P^{k,X_n}_{1|1}}}\Bigg[\sum_{t=0}^{\infty}\gamma^{t}\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg]P(\Gamma=k)\\
%         % &= P(\Gamma>n|X^n_0)\E\left[\gamma^{n+\Gamma}\left(J_{P^{\Gamma,X_n}_{P_{2|1}}}(\pi_2;P_2) - J_{P^{\Gamma,X_n}_{P_{2|2}}}(\pi_2;P_2)\right)|X_n\right].
%     \end{split}
% \end{equation}
Thus, the expected false alarm cost, conditioned on $X^n_0$ is 
\begin{equation}
    \begin{split}
        &\E[C^{\FA}_n|X^n_0] =\\
        &\E\bigg[\mathds{1}_{\{n<\Gamma\}}\bigg(\gamma^n\left(J^{\Gamma-n}_{X_n}(\pi_2;P_1) - J^{\Gamma-n}_{X_n}(\pi_1;P_1)\right)\\
        &\hspace{0.75in}+ \gamma^{\Gamma}\left(J_{P^{\Gamma-n,2|1}_{X_n}} - J_{P^{\Gamma-n,1|1}_{X_n}}\right)\bigg)|X^n_0\bigg].\\
        % &\qquad\qquad\qquad\qquad+P(\Gamma>n|X^n_0)\left(\E\left[\gamma^{\Gamma}\left(J_{P^{\Gamma-n,X_n}_{2|1}}(\pi_2;P_2) - J_{P^{\Gamma-n,X_n}_{2|2}}(\pi_2;P_2)\right)|X^n_0,\Gamma>n\right]\right)
    \end{split}
\end{equation}

\subsubsection{Expected Delay Cost}
Conditioning on $X_0^n$, the regret due to delay is 
\begin{equation}\label{eq:cond_exp_D_cost}
    \begin{split}
        &\E\left[C^{\D}_n|X^n_0\right] = \\
        &\E\Bigg[\mathds{1}_{\{\Gamma< n\}}\Bigg( \sum_{t=\Gamma}^{n-1}\gamma^t\left[c(X_t,\pi_1(X_t))-c(X'_t,\pi_2(X'_t))\right]\\
        &\hspace{0.25in}+ \sum_{t=n}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)|X^n_0\Bigg].
    \end{split}
\end{equation}
Starting with the first summation in \eqref{eq:cond_exp_D_cost}, corresponding to the time between the mode change and change declaration, we have
\begin{equation}
    \begin{split}
        &\E\left[\mathds{1}_{\{\Gamma< n\}}\Bigg( \sum_{t=\Gamma}^{n-1}\gamma^t\left[c(X_t,\pi_1(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)|X^n_0\right]\\
        &= \sum_{k=1}^{\infty}\E\Bigg[\mathds{1}_{\{k< n\}}\Bigg( \sum_{t=k}^{n-1}\gamma^t[c(X_t,\pi_1(X_t))\\
        &\hspace{0.75in}-c(X'_t,\pi_2(X'_t))]\Bigg)|X^n_0,\Gamma=k\Bigg]P(\Gamma=k|X^n_0)\\
        &= \sum_{k=1}^{\infty}\mathds{1}_{\{k< n\}}\gamma^{k}\Bigg(\sum_{t=k}^{n-1}\gamma^{t-k}c(X_t,\pi_1(X_t))\\
        &\hspace{0.1in}- \E\left[ \sum_{t=k}^{n-1}\gamma^{t-k}c(X'_t,\pi_2(X'_t))|X^n_0,\Gamma=k\right]\Bigg)P(\Gamma=k|X^n_0)\\
        &= \E\Bigg[\mathds{1}_{\{\Gamma<n\}}\gamma^{\Gamma}\Bigg(\sum_{t=\Gamma}^{n-1}\gamma^{t-\Gamma}c(X_t,\pi_1(X_t))\\
        &\hspace{1.8in}-J^{n-{\Gamma}}_{X_\Gamma}(\pi_2;P_2) \Bigg)|X^n_0\Bigg]. 
        \end{split}
    \end{equation}
For the second summation in \eqref{eq:cond_exp_D_cost}, corresponding to the time following the change declaration, we have
\begin{equation}
    \begin{split}
        &\E\left[\mathds{1}_{\{\Gamma< n\}}\Bigg( \sum_{t=n}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)|X^n_0\right]\\
        &= \sum_{k=1}^{\infty}\E\Bigg[\mathds{1}_{\{k< n\}}\Bigg( \sum_{t=n}^{\infty}\gamma^t[c(X_t,\pi_2(X_t))\\
        &\hspace{0.75in}-c(X'_t,\pi_2(X'_t))]\Bigg)|X^n_0,\Gamma=k\Bigg]P(\Gamma=k|X^n_0)\\
        &= \sum_{k=1}^{\infty}\mathds{1}_{\{k< n\}}\gamma^n\E\Bigg[\Bigg( \sum_{t=n}^{\infty}\gamma^{t-n}[c(X_t,\pi_2(X_t))\\
        &\hspace{0.75in}-c(X'_t,\pi_2(X'_t))]\Bigg)|X^n_0,\Gamma=k\Bigg]P(\Gamma=k|X^n_0)\\
        &= \E\left[\mathds{1}_{\{\Gamma<n\}}\gamma^n\left(J_{X_n}(\pi_2;P_2) - J_{P^{n-\Gamma,2|2}_{X_{\Gamma}}}(\pi_2;P_2)\right)|X^n_0\right].
    \end{split}
\end{equation}
Therefore, the expected delay term, conditioned on $X^n_0$ is 
\begin{equation}
    \begin{split}
        &\E\left[C^{\D}_n|X^n_0\right] =\\ &\E\Bigg[\mathds{1}_{\{\Gamma<n\}}\Bigg(\gamma^{\Gamma}\left(\sum_{t=\Gamma}^{n-1}\gamma^{t-\Gamma}c(X_t,\pi_1(X_t)) -J^{n-{\Gamma}}_{X_\Gamma}(\pi_2;P_2) \right)\\
        &\hspace{0.25in}+\gamma^n\left(J_{X_n}(\pi_2;P_2) - J_{P^{n-\Gamma,2|2}_{X_n}}(\pi_2;P_2)\right)\Bigg)|X^n_0\Bigg].
    \end{split}
\end{equation}

\subsubsection{Fast Mixing Approximation}
Assuming fast mixing, we have 
\begin{equation}
    \begin{split}
        &\E[C^{\FA}_n|X^n_0]\approx\\
        &\E\Bigg[\mathds{1}_{\{n<\Gamma\}}\bigg(\gamma^n\frac{1-\gamma^{(\Gamma-n)_+}}{1-\gamma}c^{\top}(\Delta_{2|1}-\Delta_{1|1})\\
        &\hspace{1in}+ \frac{\gamma^{\Gamma}}{1-\gamma}c^{\top}(\Delta_{2|2}-\Delta_{2|2})\bigg)|X^n_0\Bigg]\\
        &= \gamma^nc^{\top}(\Delta_{2|1}-\Delta_{1|1})\E\left[\mathds{1}_{\{n<\Gamma\}}\frac{1-\gamma^{(\Gamma-n)_+}}{1-\gamma}|X^n_0\right],
    \end{split}
\end{equation}
and 
\begin{equation}
    \begin{split}
        &\E\left[C^{\D}_n|X^n_0\right] \approx\\ &\E\Bigg[\mathds{1}_{\{\Gamma<n\}}\Bigg(\gamma^{\Gamma}\sum_{t=\Gamma}^{n-1}\gamma^{t-\Gamma}c(X_t,\pi_1(X_t))\,-\\
        &\hspace{0.1in}\gamma^{\Gamma}\frac{1-\gamma^{n-{\Gamma}}}{1-\gamma}c^{\top}\Delta_{2|2}+\bigg(\frac{\gamma^n}{1-\gamma}c^{\top}(\Delta_{2|2}-\Delta_{2|2})\bigg)\Bigg)|X^n_0\Bigg]\\
        &=\E\Bigg[\mathds{1}_{\{\Gamma<n\}}\gamma^{\Gamma}\Bigg(\sum_{t=\Gamma}^{n-1}\gamma^{t-\Gamma}c(X_t,\pi_1(X_t))\\
        &\hspace{1.5in}- \frac{1-\gamma^{n-{\Gamma}}}{1-\gamma}c^{\top}\Delta_{2|2}\Bigg)|X^n_0\Bigg].
    \end{split}
\end{equation}
Further assuming $\gamma = 1-\epsilon$ with $\epsilon\ll 1$, we have, for any $m\in\Zset_+$
\begin{equation}
    \lim_{\epsilon\to 0}\frac{1-\gamma^{m}}{1-\gamma} = \lim_{\epsilon\to 0}\frac{1-(1-\epsilon)^{m}}{1-(1-\epsilon)} =  m.
\end{equation}
Therefore, for $\gamma=1-\epsilon$ and sufficiently small $\epsilon$, we can further simplify our approximate costs as 
\begin{equation}
    \begin{split}
        &\E[C^{\FA}_n|X^n_0]\\
        &\hspace{0.1in}\approx (1-n\epsilon)c^{\top}(\Delta_{2|1}-\Delta_{1|1})\E\left[\mathds{1}_{\{\Gamma>n\}}(\Gamma-n)|X^n_0\right]\\
        &\hspace{0.1in}\approx c^{\top}(\Delta_{2|1}-\Delta_{1|1})\E\left[(\Gamma-n)_+|X^n_0\right]
    \end{split}
\end{equation}
and 
\begin{equation}
    \begin{split}
        &\E\left[C^{\D}_n|X^n_0\right]\approx\\ &\E\Bigg[\mathds{1}_{\{\Gamma<n\}}(1-\epsilon\Gamma)\Bigg(\sum_{t=\Gamma}^{n-1}\gamma^{t-\Gamma}c(X_t,\pi_1(X_t))\\
        &\hspace{1.75in}- c^{\top}\Delta_{2|2}(n-\Gamma)\Bigg)|X^n_0\Bigg]\approx\\
        &\E\left[\mathds{1}_{\{\Gamma<n\}}\sum_{t=\Gamma}^{n-1}\gamma^{t-\Gamma}c(X_t,\pi_1(X_t)) - c^{\top}\Delta_{2|2}(n-\Gamma)_+|X^n_0\right].
    \end{split}
\end{equation}
Therefore, the unconditional expected false alarm and delay costs under our assumption on mixing and $\gamma$ are
\begin{equation}\label{eq:exp_FA}
    \E[C^{\FA}_n] = \E\left[\E[C^{\FA}_n|X^n_0]\right] = c^{\top}(\Delta_{2|1}-\Delta_{1|1})\E[(\Gamma-n)_+].
\end{equation}
and 
\begin{equation}\label{eq:exp_D}
    \E[C^{D}_n] = \E\left[\E[C^{D}_n|X^n_0]\right] = c^{\top}(\Delta_{1|2}-\Delta_{1|1})\E[(n-\Gamma)_+].
\end{equation}
% Assuming fast mixing, we have 
% \begin{equation}
%     \begin{split}
%         &\E\left[C^{\D}_n|X^n_0\right] \approx\\ &\E\left[\mathds{1}_{\{\Gamma<n\}}\left(\gamma^{\Gamma}\left(\sum_{t=\Gamma}^{n-1}\gamma^{t-\Gamma}c(X_t,\pi_1(X_t)) -\frac{1-\gamma^{n-{\Gamma}}}{1-\gamma}c^{\top}\Delta_{2|2}\right)+\bigg(\frac{\gamma^n}{1-\gamma}c^{\top}(\Delta_{2|2}-\Delta_{2|2})\bigg)\right)|X^n_0\right]\\
%         &=\E\left[\mathds{1}_{\{\Gamma<n\}}\gamma^{\Gamma}\left(\sum_{t=\Gamma}^{n-1}\gamma^{t-\Gamma}c(X_t,\pi_1(X_t)) - \frac{1-\gamma^{n-{\Gamma}}}{1-\gamma}c^{\top}\Delta_{2|2}\right)|X^n_0\right].
%     \end{split}
% \end{equation}
Thus, overall under our assumptions on mixing times and the discount factor we have 
\begin{equation}
    \begin{split}
        % \E[Y_n] &\approx \E\left[c^{\top}(\Delta_{2|1}-\Delta_{1|1})\E\left[(\Gamma-n)_+|X^n_0\right]+c^{\top}(\Delta_{1|2}-\Delta_{2|2})\E\left[(n-\Gamma)_+|X^n_0\right]\right]\\
    \E[Y_n] &= c^{\top}(\Delta_{2|1}-\Delta_{1|1})\E\left[(\Gamma-n)_+\right]\\
    &\hspace{0.75in}+c^{\top}(\Delta_{1|2}-\Delta_{2|2})\E\left[(n-\Gamma)_+\right].
    \end{split}
\end{equation}
\eqref{eq:exp_FA} agrees with the result following from assumption that the states  of both the mode observing controller and CD based controller upon entering an $\MC(i|j)$ are distributed according to the corresponding stationary distribution $\Delta_{i|j}$. That is, if we compute 
\begin{equation}
    \begin{split}
        &\E\bigg[\mathds{1}_{\{\Gamma>n\}}\bigg(\gamma^nJ^{\Gamma-n}_{\Delta_{2|1}}(\pi_2;P_1) + \gamma^{\Gamma}J^{\Gamma-n}_{\Delta_{2|2}}(\pi_2;P_1)\\
        &\hspace{0.4in}- \left(\gamma^nJ^{\Gamma-n}_{\Delta_{1|1}}(\pi_1;P_1)) + \gamma^{\Gamma}J^{\Gamma-n}_{\Delta_{2|2}}(\pi_1;P_1))\right)\bigg)\bigg]\\
        &=\gamma^nc^{\top}(\Delta_{2|1}-\Delta_{1|1})\E\left[\mathds{1}_{\{\Gamma>n\}}\frac{1-\gamma^{\Gamma-n}}{1-\gamma}\right]\\
        &\approx (1-n\epsilon)c^{\top}(\Delta_{2|1}-\Delta_{1|1})\E\left[\mathds{1}_{\{\Gamma>n\}}(\Gamma-n)\right]\\
        &\approx c^{\top}(\Delta_{2|1}-\Delta_{1|1})\E\left[(\Gamma-n)_+\right].
    \end{split}
\end{equation}
A similar consistency holds for the expected delay cost. 
% Continuing to the expected delay term, we have 
% \begin{equation}
%     \begin{split}
%         &\E\left[\mathds{1}_{\{\Gamma\leq n\}}C^{\D}_n|X^n_0\right] = \E\left[\E\left[\mathds{1}_{\{\Gamma\leq n\}}C^{\D}_n|X^n_0,\Gamma\right]|X^n_0\right]\\
%         &= \E\Bigg[\mathds{1}_{\{n\geq \Gamma\}}\Bigg(\sum_{t=\Gamma}^{n-1}\gamma^t\left[c(X_t,\pi_1(X_t))-c(X'_t,\pi_2(X'_t))\right]\\
%         &\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad+ \sum_{t=n}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)|X^n_0\Bigg]\\
%         &= P(\Gamma\leq n|X^n_0)\E\Bigg[\gamma^{\Gamma}\left(J^{n-\Gamma}_{X_{\Gamma}}(\pi_1;P_2)-J^{n-\Gamma}_{X_{\Gamma}}(\pi_2;P_2)\right)\\
%         &\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad+ \gamma^n\left(J_{P^{n-\Gamma,X_\Gamma}_{1|2}}(\pi_2;P_2) - J_{P^{n-\Gamma,X_\Gamma}_{2|2}}(\pi_2;P_2)\right)|X^n_0\Bigg].
%     \end{split}
% \end{equation}
% Therefore, the expected cost of stopping, conditioned on $X^n_0$ is 
% \begin{equation}
%     \begin{split}
%         &\E[Y_n|X^n_0] =\\ &P(n<\Gamma|X^n_0)\E\left[\gamma^n\left(J^{\Gamma-n}_{X_n}(\pi_2;P_1) - J^{\Gamma-n}_{X_n}(\pi_1;P_1)\right) + \gamma^{\Gamma}\left(J_{P^{\Gamma-n,X_n}_{2|1}}(\pi_2;P_2) - J_{P^{\Gamma-n,X_n}_{2|2}}(\pi_2;P_2)\right)|X_n\right]\\
%         &+ P(\Gamma\leq n|X^n_0)\E\Bigg[\gamma^{\Gamma}\left(J^{n-\Gamma}_{X_{\Gamma}}(\pi_1;P_2)-J^{n-\Gamma}_{X_{\Gamma}}(\pi_2;P_2)\right)\\
%         &\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad+ \gamma^n\left(J_{P^{n-\Gamma,X_\Gamma}_{1|2}}(\pi_2;P_2) - J_{P^{n-\Gamma,X_\Gamma}_{2|2}}(\pi_2;P_2)\right)|X^n_0\Bigg].
%     \end{split}
% \end{equation}

==> cost_to_go.tex <==
When stopping in the false alarm regime, the expected cost to go, given $X_0^n$ is 

\begin{equation}\label{eq:fa_cost_to_go}
    J^{\FA}(x_0,\dots,x_n) := \E\left[J^{\Gamma-1}_{x_n}(\pi_2;P_1) + \gamma^{\Gamma}J_{P^{\Gamma-1,x_n}_{2|1}}(\pi_2;P_2)\right],
\end{equation}

That is, for $\Gamma-1$ steps $\pi_2$ will be used in mode 1, after which the mode changes (the random remaining time to the mode change is not affected by $n$ due to memorylessness). Notice that \eqref{eq:fa_cost_to_go} depends on the history only through $x_n$. When stopping in the delay regime at time $n$, the cost to go is 
\begin{equation}\label{eq:delay_cost_to_go}
    % J^{\D}(x_0,\dots,x_n) = \E\left[J_{P^{n-\Gamma,x_{\Gamma}}_{1|2}}(\pi_2;P_2)\right],
    J^{\D}(x_0,\dots,x_n) = \E\left[J_{x_n}(\pi_2;P_2)\right],
\end{equation}
Note that for the delay case, the cost to go when switching to $\pi_2$, given the system is in mode 2, will be affected by the initial distribution induced by the delay incurred. Since the (random) mode change is unobserved, and could have occurred at any point prior to $n$, the entire history of states needs to be retained in order to compute the expectation in \eqref{eq:delay_cost_to_go}. Summing these terms together, we have that the expected cost to go of stopping at time $n$ is 
\begin{equation}
\begin{split}
    J^{\text{S}}(x_0,\dots,x_n,p_n) &= (1-p_n)\cdot J^{\FA}(x_0,\dots,x_n)\\
    &\hspace{0.5in}+p_n\cdot J^{\D}(x_0,\dots,x_n),
\end{split}
\end{equation}
where 
\begin{equation}
    p_n = P(\Gamma\leq n|X^n_0).
\end{equation}
On the other hand, continuing in our setting means using policy $\pi_1$ for another step, and then incurring the subsequent expected cost to go:
\begin{equation}
    \begin{split}
        J^{\text{C}}&(x_0,\dots,x_n,p_n) = c(x_n,\pi_1(x_n))\\
        &+ \E\left[J(x_0,\dots,x_n,X_{n+1},p_{n+1})|x_0,\dots,x_n,p_n\right],
    \end{split}
\end{equation}
where 
\begin{equation}\label{eq:exact_cost_to_go}
    \begin{split}
        &J(x_0,\dots,x_n,p_n) =\\
        &\hspace{0.25in}\min\left\{J^{\text{S}}(x_0,\dots,x_n,p_n),J^{\text{C}}(x_0,\dots,x_n,p_n)
    \right\} 
    \end{split}
\end{equation}

To avoid explicit dependence on the entire observation history, we will assume fast mixing of all Markov chains in our setting. Using the argument presented in the following section, we can bound the error incurred under our approximating assumption.

\nate{Need to streamline link between complicated expected costs and goal of deriving stopping policy.}

\nate{Describe mixing process.}

==> formalizing_regret.tex <==
Let $\v{X} = \{X_t\}_{t\geq0}$ and $\v{X}'=\{X'_t\}_{t\geq 0}$ denote the sequence of state observations generated by the change detection (CD) based and mode observing controllers, respectively, under the same random change point $\Gamma$. Note that $X_t = X'_t$ for $t\leq \min\{\tau,\Gamma\}$, i.e. the state trajectories of the CD and mode observing controllers will always agree prior to the change point, or the time at which the CD controller switches to $\pi_2$, whichever is earlier. The random regret over the infinite horizon, i.e., the difference in long term costs under the two controllers, when the CD controller switches at $\tau=n$ is
\begin{equation}\label{eq:random_regret}
    \begin{split}
        % &Y_n = \mathds{1}_{\{n<\Gamma\}}\Bigg(\sum_{t=0}^{n-1}\gamma^t\left[c(X_t,\pi_1(X_t))-c(X'_t,\pi_1(X'_t))\right]\\
        % &\hspace{0.75in}+ \sum_{t=n}^{\Gamma-1}\gamma^t\left[c(X_t,\pi_2(X_t)) - c(X'_t,\pi_1(X'_t))\right]\\
        % &\hspace{0.75in}+ \sum_{t=\Gamma}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)\\
        % &\hspace{0.25in}+ \mathds{1}_{\{n> \Gamma\}}\Bigg(\sum_{t=0}^{\Gamma-1}\gamma^t\left[c(X_t,\pi_1(x_t)) - c(X'_t,\pi_1(X'_t))\right]\\
        % &\hspace{0.75in}+ \sum_{t=\Gamma}^{n-1}\gamma^t\left[c(X_t,\pi_1(X_t))-c(X'_t,\pi_2(X'_t))\right]\\
        % &\hspace{0.75in}+ \sum_{t=n}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)\\
    %%%%%%
        &R_n(\v{X},\v{X}')
        \\ 
        &:= \mathds{1}_{\{n<\Gamma\}}\Bigg(\sum_{t=n}^{\Gamma-1}\gamma^t\left[c(X_t,\pi_2(X_t)) - c(X'_t,\pi_1(X'_t))\right]\\
        &\hspace{0.6in}+ \sum_{t=\Gamma}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg)\\
        &\hspace{0.1in}+ \mathds{1}_{\{n> \Gamma\}}\Bigg( \sum_{t=\Gamma}^{n-1}\gamma^t\left[c(X_t,\pi_1(X_t))-c(X'_t,\pi_2(X'_t))\right]\\
        &\hspace{0.6in}+ \sum_{t=n}^{\infty}\gamma^t\left[c(X_t,\pi_2(X_t))-c(X'_t,\pi_2(X'_t))\right]\Bigg).
        % &\hspace{0.1in}= R^{\FA}_n +R^{\D}_n,
    \end{split}
\end{equation}
% where $R^{\FA}_n$ and $R^{\D}_n$ denote the regret associated with false alarm and delay, respectively, when switching the controller at time $n$. 
Upon switching controller at time $n$, the expected regret is given by 
\begin{equation}
    r_n := \E\left[R_n(\v{X},\v{X}')|X^n_0\right],
\end{equation}
conditioned on the observations up to time $n$. We seek to identify a causal switching rule $\tau$ that defines an extended integer-valued random variable, adapted to the filtration $ \{\sigma(X_1,\dots,X_n)\}$, generated by the stochastic process. Let $r_{\tau}$ denote the expected regret at the switching time generated by $\tau$, i.e. $r_{\tau}=r_n$ when $\tau$ selects $n$. Defining $\Scal$ as the set of all causal switching policies, we aim to solve
\begin{equation}\label{eq:stopping_obj}
    \min_{\tau\in\Scal}\,\,\Rcal(\tau):= \E[r_{\tau}],
    %= \min_{\tau\in\Scal}\,\,\E[r_{\tau}]
\end{equation}
where 
% In particular, given a sequence of observations $\tau$ determines a random time $N(\tau)$ at which stopping occurs. 
% \begin{equation}
%     \min_{\tau\in \Scal}\,\,\E[R_{N(\tau)}],
% \end{equation}
% over the set of causal stopping rules $\Scal$. Such rules comprise decisions to switch the controller, and are adapted to the same filtration.

% Stopping at time $n$, the actual value of $R_n$ is not known. However, as the decision to stop at time $n$ may depend on $X_0^n$, we may replace the random regret sequence $R_0,R_1,\dots,R_{\infty}$ with a sequence of regret functions, given by the conditional expectation 
% \begin{equation}
%     r_n \equiv r_n(X^n_0) := \E\left[R_n(\v{X},\v{X}')|X^n_0\right].
% \end{equation}
% Any stopping rule $\tau$ for the sequence $R_0,R_1,\dots,R_{\infty}$ will yield the same expected regret for the sequence $r_0,r_1,\dots,r_{\infty}$. We analogously define $r^{\FA}_n$ and $r^{\D}_n$. 
% Therefore, defining $$\Rcal_{\tau}:=\E[r_{\tau}]$$, we can instead solve the following problem
% \begin{equation}\label{eq:stopping_obj}
%     \min_{\tau\in\Scal}\,\,\Rcal_{\tau}:= \E[r_{\tau}]. 
%     %= \min_{\tau\in\Scal}\,\,\E[r_{\tau}]
% \end{equation}
% and associated components $r^{\FA}_n$ and $r^{\D}_n$ defined analogously. 
% \textcolor{blue}{Figure here showing different cases.}
\begin{figure}[h]\label{fig:earlydetect}
\includegraphics[width=8cm]{Figures/FalseAlarm.png}
\centering
\caption{Early cry for mode change.}
\end{figure}
\begin{figure}[h]\label{fig:earlydetect}
\includegraphics[width=8cm]{Figures/Delay.png}
\centering
\caption{Delay in mode change detection.}
\end{figure}
% Here, we assume that a prior on the change point is given. In particular, we assume that the mode transition occurs at time $\Gamma=k\geq 1$ with a probability $\rho(1-\rho)^{k-1}$, where $\rho \in (0,1)$.

% Therefore, given our restriction to switching policies, we have the following objective 
% \begin{equation}\label{eq:stopping_obj}
%     \min_{\tau\in \Scal}\,\, \E[r_{\tau}(\v{X},\v{X}')] =: \Rcal_{\tau},
%     %= \min_{\tau\in \Scal}\,\,\E\left[R^{\FA}_{\tau} + R^{\D}_{\tau}\right],
% \end{equation}
% where $\Scal$ is the set of of stopping times for the sequence $\v{X}$ i.e., for each $\tau\in\Scal$, the event $\{\tau\leq n\}$ belongs to the sigma-algebra $\Fcal^X_n=\sigma(X_0,\dots,X_n)$. %The expectation in \eqref{eq:stopping_obj} is taken with respect to the chosen stopping rule $\tau$, change point $\Gamma$, and environment dynamics as described by $P_1$ and $P_2$.
% Now, we have
\begin{equation}\label{eq:stopping_obj_cond}
    \begin{split}
        % \Rcal_{\tau}  &= \E\left[\E\left[r_{\tau}|\v{X}\right]\right]\\
        % &= \E\left[\sum_{n=0}^{\infty}\E\left[r_n|\v{X}\right]P(\tau=n|\v{X})\right]\\
        % &= \E\left[\sum_{n=0}^{\infty}\E\left[r_n|X_0^n\right]P(\tau=n|X_0^n)\right]\\
        \Rcal(\tau)&= \E\left[\sum_{n=0}^{\infty}r_nP(\tau=n|X_0^n)\right]\\
        &= \E\left[\sum_{n=0}^{\infty}(r^{\FA}_n + r^{\D}_n)P(\tau=n|X_0^n)\right],
        % &= \E\left[\sum_{n=0}^{\infty}\E[R_n(X_0^n,|X_0^n,\tau=n]P(\tau=n|X_0^n)\right]
    \end{split}
\end{equation}
$r^{\FA}_n$ and $r^{\D}_n$ denote the expected regret due to a false alarm or delay in switching at time $n$, and are defined as the expectation of the terms involving  $\mathds{1}_{\{n<\Gamma\}}$ and $\mathds{1}_{\{n>\Gamma\}}$ in \eqref{eq:random_regret}, respectively, conditioned on $X^n_0$.

% \nate{define $r^{\FA}_n$ and $r^{\D}_n$}
In order to further analyze the expected regret in \eqref{eq:stopping_obj}, we need to introduce additional notation. %Let $\Pcal$ denote the set of distributions over the state space $\Xset$. 
$J^m_{i|j}(Q)$ denotes the expected $m$ step horizon cost, when initial state is distributed according to $Q$ and policy $\pi_i$ is used under system mode $j$, for $i,j=1,2$. If the initial state $X$ is given, we write $J^m_{i|j}(\delta_X)$, where $\delta_X$ is the measure concentrated at $X$. %In either case, when $m=\infty$, we drop the superscript, e.g. $J_{i|j}(Q) := J^{\infty}_{i|j}(Q)$. Lastly, we denote as %$P^{m,i|j}_{X} = P(X,\pi_i,j,m)$ 
Let $P^{m}_{i|j}(X)$ be the $m$ step probability distribution, given that the system started in state $X$, and policy $\pi_i$ was used in system mode $j$. 
Additionally, we denote the stationary state distribution arising from the use of policy $\pi_i$ in mode $j$, for $i,j=1,2$ as $\Delta_{i|j}$, and the associated Markov chain as $\Mcal_{i|j}$. 
% $\MC(\Delta_{i|j})$. 
% \nate{Keep $\infty$ superscript.}

With this notation in hand, we can give expected regret terms corresponding to the false alarm and delay cases, conditioned on the history of state observations until time $n$. We further develop approximations of See Appendix \ref{app:expected_regret} for a detailed derivation. 

\begin{proposition}
% Conditioned on the state observation history $X_0^n$, the expected regret due to false alarm and delay is given by
The following assertions hold:
\begin{equation}\label{eq:prop_r_FA}
    \begin{split}
        r^{\FA}_n & = \E\bigg[\mathds{1}_{\{n<\Gamma\}}\bigg(\gamma^n\left(J^{\Gamma-n}_{2|1}(\delta_{X_n}) - J^{\Gamma-n}_{1|1}(\delta_{X_n})\right)\\
        &\hspace{0.05in} + \gamma^{\Gamma}\left(J^{\infty}_{2|2}\left(P^{\Gamma-n}_{2|1}(X_n)\right) - J^{\infty}_{2|2}\left(P^{\Gamma-n}_{1|1}(X_n)\right)\right)\bigg)|X^n_0\bigg],\\
    \end{split}
\end{equation}
\begin{equation}\label{eq:prop_r_D}
    \begin{split}
        &r^{\D}_n = \E\Bigg[\mathds{1}_{\{\Gamma<n\}}\Bigg(\gamma^{\Gamma}\left(\sum_{t=\Gamma}^{n-1}\gamma^{t-\Gamma}c(X_t,\pi_1(X_t)) -J^{n-{\Gamma}}_{2|2}(\delta_{X_{\Gamma}}) \right)\\
        &\hspace{0.6in}+\gamma^n\left(J^{\infty}_{2|2}(\delta_{X_n}) - J^{\infty}_{2|2}(P^{n-\Gamma}_{2|2}(\delta_{X_{\Gamma}}))\right)\Bigg)|X^n_0\Bigg].
    \end{split}
\end{equation}
\end{proposition}

Expressions \eqref{eq:prop_r_FA} and \eqref{eq:prop_r_D} provide further insight into the sources of expected regret when stopping at time $n$. In the false alarm scenario, the CD based controller will erroneously use $\pi_2$ in mode 1 for $\Gamma-n$ time steps. The regret incurred during this period consists of a transient component as $\Mcal_{2|1}$ and $\Mcal_{1|1}$ mix to $\Delta_{2|1}$ and $\Delta_{1|1}$, as well as a steady state component due to the difference between $\Delta_{2|1}$ and $\Delta_{1|1}$. Similar transient and steady state components will generally arise when either the mode changes, or the CD based controller declares a change.

Continuing in \eqref{eq:prop_r_FA}, there is a discrepancy between the distributions of the states $X_{\Gamma}$ and $X'_{\Gamma}$ due to the difference in control policies used by the CD and mode observing controllers for $\Gamma-n$ steps. 
% In turn, this causes a difference in the long term costs incurred once both controllers are using $\pi_2$ in mode 2, as the $\MC(\Delta_{2|2}$ will take time to mix to its stationary distribution. 

Similarly, in the delayed detection scenario, the first term inside the expectation in \eqref{eq:prop_r_D} describes the regret due to the CD controller using $\pi_1$ for $n-\Gamma$ steps after the mode change occurs. Again, this discrepancy causes a difference in the distribution of states $X_n$ and $X'_n$, and thus the expected long term costs over the remaining horizon in mode 2. 

In terms of selecting a stopping rule, the form of \eqref{eq:prop_r_FA} and \eqref{eq:prop_r_D} introduce substantial difficulties. It can be shown that the optimal stopping rule can be obtained from the solution to the Bellman equation 
\begin{equation}
\begin{split}
    &V(X^n_0) =\\ &\min\left\{\left(J^{\infty}_{2|2}\left(P^{\Gamma-n}_{2|1}(X_n)\right) - J^{\infty}_{2|2}\left(P^{\Gamma-n}_{1|1}(X_n)\right)\right)\bigg)\right\}
\end{split}
\end{equation}
% Typically, optimal or near optimal stopping rules select a stopping time $N$ according to 
% \begin{equation}\label{eq:1-sla}
%     N = \min\{n\geq 0\,:\,r_n\leq \E\left[r_{n+1}|X_0^n\right]\}. 
% \end{equation}
% \nate{Is this correct? Compare with Shiryaev case.}
The rule in \eqref{eq:1-sla} incurs explicit evaluation of \eqref{eq:prop_r_FA} and \eqref{eq:prop_r_D}, requiring computation of finite and infinite horizon expected discounted costs, which often do not yield closed form expressions, requiring numerical estimation. As the change point $\Gamma$ is not observed, these discounted costs must be computed over ranges of potential values for $\Gamma$. Further, as \eqref{eq:prop_r_D} includes terms involving $X_{\Gamma}$, i.e., as the change point may have occurred at any time prior to $n$, the entire history of state observations must be retained.

In light of these difficulties, we now develop an approximation to $r_n$, which in turn yields a more tractable approximation of the expected regret minimization problem \eqref{eq:stopping_obj}. 

\bose{Talk about the actual dynamics in each possible error situations. Talk about how it mixes and why this introduces a difficulty in solving the problem. Introduce the notion of approximate regret minimization.}

\nate{Classic DP approach not possible due to \begin{itemize}
    \item Maintaining history
    \item No closed for for $J$
    \item Mixing 
    \item State dependency
\end{itemize}
Contrast with classic Shiryaev case}

% \subsection{Cost To Go Functions}
% \input{cost_to_go.tex}
% \section{Formalizing Regret Analysis}

% Given our choice of the benchmark and the switching algorithm, we now characterize the regret. There are two ways that one loses performance using a CD algorithm. You declare a mode change too early or too late. We tackle the two cases separately. In the sequel, assume that mode change happens at $\Gamma=k$, while the algorithm declares a change at $t=n$.
% \begin{figure}[h]\label{fig:earlydetect}
% \includegraphics[width=8cm]{Figures/FalseAlarm.png}
% \centering
% \caption{Early cry for mode change.}
% \end{figure}
% \paragraph{Early cry for mode change ($n < k$).}
% When the controller switches too early, we operate the MDP with $P_1$ as the transition kernel with $\pi_2$ for times $t=n, n+1, \ldots, k-1$. %Then, we switch it to $\pi_2$. 
% If $k-n$ is sufficiently large, then the controlled Markov chain with $P_1$ and $\pi_2$ will mix well and converge to its stationary distribution. Call this distribution $\Delta_{2|1}$. Assume that the chain is such that it admits a unique stationary distribution with positive support on all states. When the mode change finally occurs at time $k$, again assume that the controlled Markov chain under $P_2$ and $\pi_2$ admits a unique invariant distribution $\Delta_{2|2}$ with positive probability on all states. In the early cry scenario, the cost borne by the reference, mode observing controller is
% \begin{align}
%     J^*(X_n) &= \E^{P_1,\pi_1}\left[\sum_{t=n}^{k-1}\gamma^{t-n}c(X_t,U_t)|X_n\right] + \gamma^{k-n}\E^{P_2,\pi_2}\left[\sum_{t=k}^{\infty}\gamma^{t-k}c(X_t,U_t)|X_n\right],
% \end{align}
% where $\Eset^{P_i,\pi_j}$ for $i,j\in 1,2$ indicates that $X_t\sim P_i(\cdot|x_{t-1},u_{t-1})$ and $U_t\sim\pi(\cdot|X_t)$ for each $X_t$ and $U_t$ within the expectation. 
% The cost borne by the CD algorithm from time $t=n$ onwards is given by 
% \begin{align}\label{eq:FA_cost}
%     % \E_{X_t \sim P_1(\cdot|x_{t-1}, u_{t-1}), U_t \sim \pi_2(\cdot | X_t)}\left[ \sum_{t=N}^{t=T-1} \gamma^{t-N} c(X_t, U_t)  + \gamma^{T-N} J(X_T; P_2, \pi_2) \vert  X_N \right].
%     J(X_n) &= \underbrace{\E^{P_1,\pi_2}\left[ \sum_{t=n}^{k-1} \gamma^{t-n} c(X_t, U_t)|X_n\right]}_{J_1(X_n)} + \gamma^{k-n}\underbrace{\E^{P_2,\pi_2}\left[\sum_{t=k}^{\infty}\gamma^{t-k}c(X_t,U_t)|X_n\right]}_{J_2(X_n)}.
% \end{align}
% We now consider the expectation of \eqref{eq:FA_cost} when $X_n$ is distributed according to $\Delta_{1|1}$:
% $$\E_{X_n\sim \Delta_{1|1}}\left[J(X_n)\right] = \E_{X_n\sim \Delta_{1|1}}\left[J_1(X_n)\right] + \gamma^{k-n}\E_{X_n\sim \Delta_{1|1}}\left[J_2(X_n)\right].$$

% $J_1(X_n)$, the first term in \eqref{eq:FA_cost} has a mixing component and a portion of $J(X_n; P_1, \pi_2)$ over the horizon $(k-n)$. Regarding the latter, suppose that $X_n$ is distributed according to $\Delta_{2|1}$. Then
% \begin{align}\label{eq:inf_finite_dev1}
%     &\E_{X_n\sim \Delta_{2|1}}\left[J(X_n;P_1,\pi_2)\right] = \E_{X_n\sim \Delta_{2|1}}\left[\E^{P_1,\pi_2}\left[\sum_{t=n}^{\infty}\gamma^{t-n}c(X_t,U_t)|X_n\right]\right]\\
%     \label{eq:inf_finite_dev2}
%     &= \E_{X_n\sim \Delta_{2|1}}\left[\E^{P_1,\pi_2}\left[\sum_{t=n}^{k-1}\gamma^{t-n}c(X_t,U_t)+\sum_{t=k}^{\infty}\gamma^{t-n}c(X_t,U_t)|X_n\right]\right]\\
%     \label{eq:inf_finite_dev3}
%     &= \E_{X_n\sim \Delta_{2|1}}\left[\E^{P_1,\pi_2}\left[\sum_{t=n}^{k-1}\gamma^{t-n}c(X_t,U_t)|X_n\right]\right]+\E_{X_k\sim \Delta_{2|1}}\left[\E^{P_1,\pi_2}\left[\sum_{t=k}^{\infty}\gamma^{t-n}c(X_t,U_t)|X_k\right]\right]\\
%     \label{eq:inf_finite_dev4}
%     &= \E_{X_n\sim \Delta_{2|1}}\left[\E^{P_1,\pi_2}\left[\sum_{t=n}^{k-1}\gamma^{t-n}c(X_t,U_t)|X_n\right]\right]+\gamma^{k-n}\E_{X_n\sim \Delta_{2|1}}\left[J(X_n;P_1,\pi_2)\right],
% \end{align}
% so that 
% \begin{align}\label{eq:FA_finite_cost}
%     \E_{X_n\sim \Delta_{2|1}}\left[\E^{P_1,\pi_2}\left[\sum_{t=n}^{k-1}\gamma^{t-n}c(X_t,U_t)|X_n\right]\right] &= (1-\gamma^{k-n})\E_{X_n\sim \Delta_{2|1}}\left[J(X_n;P_1,\pi_2)\right].
% \end{align}
% Let $\MC(P)$ denote the Markov chain associated with stationary distribution $P$. The term in \eqref{eq:FA_finite_cost} represents the cost of switching from policy $\pi_1$ to $\pi_2$ $k-n$ steps early, assuming $\MC(\Delta_{2|1})$ mixes to its stationary distribution immediately. 

% In the following discussion, we will denote costs associated with mixing from one stationary distribution $P$ to another $Q$ as $\Ecal(P,Q)$. As $X_n$ is assumed to be distributed according to $\Delta_{1|1}$, and in general $\MC(\Delta_{2|1})$ will have a positive mixing time, we may write 
% \begin{align}
%     \E_{X_n\sim\Delta_{1|1}}\left[J_1(X_n)\right] = \Ecal(\Delta_{1|1},\Delta_{2|1}) + (1-\gamma^{k-n})\E_{x\sim \Delta_{2|1}}\left[J(x;P_1,\pi_2)\right].
% \end{align}
% % Denote the unnormalized, discounted occupancy measure assocated with $\Delta_{i|j}$ as $\eta_{i|j}$, i.e.
% % $$\eta_{i|j}(s,a) := \E^{P_j,\pi_i}\left[\sum_{t=0}^{\infty}\gamma^t\delta_{s,a}(s_t,a_t)\right].$$
% Since $\E_{x\sim \Delta_{2|1}}\left[J(x;P_1,\pi_2)\right]= \langle\Delta_{2|1},c\rangle/(1-\gamma)$, we have
% \begin{align}
%     \E_{X_n\sim\Delta_{1|1}}\left[J_1(X_n)\right] = \Ecal(\Delta_{1|1},\Delta_{2|1}) +\left(\frac{1-\gamma^{k-n}}{1-\gamma}\right)\langle\Delta_{2|1},c\rangle.
% \end{align}
% When $\gamma\approx 1$, i.e., when $\gamma=1-\epsilon$ with $\epsilon\ll 1$, we have that $\gamma^{k-n} = (1-\epsilon)^{k-n} \approx 1-(k-n)\epsilon$, so that 
% \begin{align}
%     \E_{X_n\sim\Delta_{1|1}}\left[J_1(X_n)\right] \approx \Ecal(\Delta_{1|1},\Delta_{2|1}) + (k-n)\langle \Delta_{2|1},c\rangle.
% \end{align}
% Following a similar development, we have that 
% \begin{equation}
%     \E_{X_n\sim\Delta_{1|1}}\left[J_2(X_n)\right] \approx (1-(k-n)\epsilon)\left(\Ecal(\Delta_{2|1},\Delta_{2|2}) +\frac{\langle \Delta_{2|2},c\rangle}{\epsilon} \right),
% \end{equation}
% and 
% \begin{equation}
%     \begin{split}
%         \E_{X_n\sim\Delta_{1|1}}[J(X_n)] \approx  \Ecal(\Delta_{1|1}&,\Delta_{2|1}) + (k-n)\langle\Delta_{2|1},c\rangle+ (1-(k-n)\epsilon)\left(\Ecal(\Delta_{2|1},\Delta_{2|2}) +\frac{\langle \Delta_{2|2},c\rangle}{\epsilon} \right).
%     \end{split}
% \end{equation}
% Similar analysis of $\E_{X_N\sim\Delta_{1|1}}[J^*(X_n)]$ gives 
% \begin{equation}
%     \E_{X_n\sim\Delta_{1|1}}[J^*(X_n)]\approx (k-n)\langle \Delta_{1|1},c\rangle + (1-(k-n)\epsilon)\left(\Ecal(\Delta_{1|1},\Delta_{2|2}) + \frac{\langle\Delta_{2|2},c\rangle}{\epsilon}\right).
% \end{equation}
% Letting $h = (k-n)_+$ and denoting the expected regret due to false alarm of length $h$ as $R^{\FA}(h)$, we have 
% \begin{equation}
% \begin{split}
%     &R^{\FA}(h) \approx \Ecal(\Delta_{1|1},\Delta_{2|1}) +h\langle\Delta_{2|1}-\Delta_{1|1},c\rangle +  (1-\epsilon h)(\Ecal(\Delta_{2|1},\Delta_{2|2}) - \Ecal(\Delta_{1|1},\Delta_{2|2})).
% \end{split}
% \end{equation}
% Assuming that mixing effects are negligible, we have 
% \begin{equation}
% \begin{split}
%     &R^{\FA}(h) \approx h\langle\Delta_{2|1}-\Delta_{1|1},c\rangle.
% \end{split}
% \end{equation}



% % If this horizon is long enough, then we can drop the mixing term and approximate the $(T-N)$-length portion of the infinite horizon cost $J(X_N; P_1, \pi_2)$ as linear in $T-N$.
% % \begin{align}
% %     J = J(H) + \gamma^H J \implies J(H) \approx  (1-\gamma^H ) J \approx H (1-\gamma) J.
% % \end{align}

% \begin{figure}[h]\label{fig:earlydetect}
% \includegraphics[width=8cm]{Figures/Delay.png}
% \centering
% \caption{Delay in mode change detection.}
% \end{figure}
% \paragraph{Late call on mode change ($k < n$).} In contrast to the previous section, when the controller switches too late, we operate the MDP with $P_2$ as the transition kernel with $\pi_1$ for times $=k,k+1,\dots,k-1$. Similar to the previous case, we assume that $n-k$ is sufficiently large to allow $\MC(\Delta_{1|2})$ to mix well and converge to its stationary distribution. In this situation, the cost borne by the CD algorithm from time $t=k$ onwards is 

% \begin{align}\label{eq:delay_cost}
%     % \E_{X_t \sim P_1(\cdot|x_{t-1}, u_{t-1}), U_t \sim \pi_2(\cdot | X_t)}\left[ \sum_{t=N}^{t=T-1} \gamma^{t-N} c(X_t, U_t)  + \gamma^{T-N} J(X_T; P_2, \pi_2) \vert  X_N \right].
%     J(X_k) &= \underbrace{\E^{P_2,\pi_1}\left[ \sum_{t=k}^{t=n-1} \gamma^{t-k} c(X_t, U_t)|X_k\right]}_{J_1(X_k)} + \gamma^{n-k}\underbrace{\E^{P_2,\pi_2}\left[\sum_{t=n}^{\infty}\gamma^{t-k}c(X_t,U_t)|X_k\right]}_{J_2(X_k)}.
% \end{align}
% Following the development of  \eqref{eq:inf_finite_dev1}-\eqref{eq:inf_finite_dev4}, we may write 
% \begin{align}\label{eq:delay_finite_cost}
%     \E_{X_k\sim \Delta_{1|2}}\left[\E^{P_2,\pi_1}\left[\sum_{t=k}^{n-1}\gamma^{t-k}c(X_t,U_t)|X_k\right]\right] &= (1-\gamma^{n-k})\E_{X_k\sim \Delta_{1|2}}\left[J(X_k;P_2,\pi_1)\right].
% \end{align}
% Again under the assumption that $\gamma=1-\epsilon$ with $\epsilon\ll 1$, we have 
% \begin{align}
%     \E_{X_k\sim\Delta_{1|2}}\left[J_1(X_k)\right] \approx \Ecal(\Delta_{1|1},\Delta_{1|2}) + (n-k)\langle\Delta_{1|2},c\rangle,
% \end{align}
% and 
% \begin{equation}
%     \E_{X_k\sim\Delta_{1|2}}\left[J_2(X_k)\right] \approx (1-(n-k)\epsilon)\left(\Ecal(\Delta_{1|2},\Delta_{2|2}) +\frac{\langle \Delta_{2|2},c\rangle}{\epsilon} \right), 
% \end{equation}
% so that 
% \begin{equation}
%     \begin{split}
%         \E_{X_k\sim\Delta_{1|2}}[J(X_k)] \approx  \Ecal(\Delta_{1|1}&,\Delta_{1|2}) + (n-k)\langle \Delta_{1|2},c\rangle+ (1-(n-k)\epsilon)\left(\Ecal(\Delta_{1|2},\Delta_{2|2}) +\frac{\langle \Delta_{2|2},c\rangle}{\epsilon} \right).
%     \end{split}
% \end{equation}
% Now letting $d=(n-k)_+$, and denoting the expected regret due to a detection delay of length $d$ as $R^{\D}(d)$, we have 
% \begin{equation}
%     R^{\D}(d) \approx \Ecal(\Delta_{1|1},\Delta_{1|2}) + d\langle\Delta_{1|2}-\Delta_{2|2},c\rangle + (1-\epsilon D)(\Ecal(\Delta_{1|2},\Delta_{2|2}) - \Ecal(\Delta_{1|1},\Delta_{2|2})).
% \end{equation}
% Again assuming that mixing affects are negligible, we have that 
% \begin{equation}
%     R^{\D}(d)\approx d\langle\Delta_{1|2}-\Delta_{2|2},c\rangle.
% \end{equation}
